Integral Identities for the boundary of a convex body

We present the multidimensional versions of the Pleijel and Ambartzumian--Pleijel identities. We also obtain the generalization of both the Blaschke--Petkantschin and Z\"ahle formulae considering the case when some points are chosen inside the convex body and some on the boundary. Moreover, a version of the Z\"ahle formula for the polytopes is derived.

==> def.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}% amstex ?
\usepackage{amsthm}
\usepackage{amssymb,bbm}%
\usepackage[numbers, square]{natbib}



%Theorems***************************************
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{convention}[theorem]{Convention}
\newtheorem{claim}[theorem]{Claim}
\makeindex
\makeglossary

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\Sd}{\mathbb{S}^{d-1}}
\newcommand{\bV}{\mathbb{\hspace{-.07mm}V\hspace{-.2mm}}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\E}{\mathbb E\,}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\s}{\mathbb{S}}
\newcommand{\B}{\mathbb{B}}
\renewcommand{\P}{\mathbb{P}}
%\mathrm commands
\newcommand{\Var}{\mathop{\mathrm{Var}}\nolimits}
\newcommand{\Int}{\mathop{\mathrm{int}}\nolimits}
\newcommand{\cl}{\mathop{\mathrm{cl}}\nolimits}
\newcommand{\bd}{\mathop{\mathrm{bd}}\nolimits}
\newcommand{\relint}{\mathop{\mathrm{relint}}\nolimits}
\newcommand{\relcl}{\mathop{\mathrm{relcl}}\nolimits}
\newcommand{\relbd}{\mathop{\mathrm{relbd}}\nolimits}
\newcommand{\Vol}{\mathop{\mathrm{Vol}}\nolimits}
\newcommand{\supp}{\mathop{\mathrm{supp}}\nolimits}
\newcommand{\Cov}{\mathop{\mathrm{Cov}}\nolimits}
\newcommand{\conv}{{\mathrm{conv}}}
\newcommand{\cone}{\mathop{\mathrm{cone}}\nolimits}
\newcommand{\spec}{\mathop{\mathrm{spec}}\nolimits}
\newcommand{\pos}{\mathop{\mathrm{pos}}\nolimits}
\newcommand{\lin}{\mathop{\mathrm{lin}}\nolimits}
\newcommand{\aff}{\mathop{\mathrm{aff}}\nolimits}
\newcommand{\dist}{\mathop{\mathrm{dist}}\nolimits}
\newcommand{\diam}{\mathop{\mathrm{diam}}\nolimits}
\newcommand{\Span}{\mathop{\mathrm{span}}\nolimits}
\newcommand{\rank}{\mathop{\mathrm{rank}}\nolimits}
\newcommand{\codim}{\mathop{\mathrm{codim}}\nolimits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\nolimits}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\nolimits}

\newcommand{\eqdistr}{\stackrel{d}{=}}
\newcommand{\todistr}{\overset{d}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toweak}{\overset{w}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toprobab}{\overset{P}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toas}{\overset{a.s.}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\ton}{\overset{}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\tosquare}{\stackrel{L^2}{\to}}
\newcommand{\bsl}{\backslash}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bu}{\mathbf{u}}


\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bEta}{\boldsymbol{\eta}}
\newcommand{\dd}{{\,\rm d}}

\newcommand{\stirling}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand{\stirlingsec}[2]{\genfrac{\{}{\}}{0pt}{}{#1}{#2}}

\newcommand{\given}{\,|\,}
\newcommand{\bgiven}{\,\big|\,}



==> def__1_.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}% amstex ?
\usepackage{amsthm}
\usepackage{amssymb,bbm}%
\usepackage[numbers, square]{natbib}



%Theorems***************************************
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}{Example}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{convention}[theorem]{Convention}
\newtheorem{claim}[theorem]{Claim}
\makeindex
\makeglossary

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\Sd}{\mathbb{S}^{d-1}}
\newcommand{\bV}{\mathbb{\hspace{-.07mm}V\hspace{-.2mm}}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\E}{\mathbb E\,}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\s}{\mathbb{S}}
\newcommand{\B}{\mathbb{B}}
\renewcommand{\P}{\mathbb{P}}
%\mathrm commands
\newcommand{\Var}{\mathop{\mathrm{Var}}\nolimits}
\newcommand{\Int}{\mathop{\mathrm{int}}\nolimits}
\newcommand{\cl}{\mathop{\mathrm{cl}}\nolimits}
\newcommand{\bd}{\mathop{\mathrm{bd}}\nolimits}
\newcommand{\relint}{\mathop{\mathrm{relint}}\nolimits}
\newcommand{\relcl}{\mathop{\mathrm{relcl}}\nolimits}
\newcommand{\relbd}{\mathop{\mathrm{relbd}}\nolimits}
\newcommand{\Vol}{\mathop{\mathrm{Vol}}\nolimits}
\newcommand{\supp}{\mathop{\mathrm{supp}}\nolimits}
\newcommand{\Cov}{\mathop{\mathrm{Cov}}\nolimits}
\newcommand{\conv}{{\mathrm{conv}}}
\newcommand{\cone}{\mathop{\mathrm{cone}}\nolimits}
\newcommand{\spec}{\mathop{\mathrm{spec}}\nolimits}
\newcommand{\pos}{\mathop{\mathrm{pos}}\nolimits}
\newcommand{\lin}{\mathop{\mathrm{lin}}\nolimits}
\newcommand{\aff}{\mathop{\mathrm{aff}}\nolimits}
\newcommand{\dist}{\mathop{\mathrm{dist}}\nolimits}
\newcommand{\diam}{\mathop{\mathrm{diam}}\nolimits}
\newcommand{\Span}{\mathop{\mathrm{span}}\nolimits}
\newcommand{\rank}{\mathop{\mathrm{rank}}\nolimits}
\newcommand{\codim}{\mathop{\mathrm{codim}}\nolimits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\nolimits}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\nolimits}

\newcommand{\eqdistr}{\stackrel{d}{=}}
\newcommand{\todistr}{\overset{d}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toweak}{\overset{w}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toprobab}{\overset{P}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\toas}{\overset{a.s.}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\ton}{\overset{}{\underset{n\to\infty}\longrightarrow}}
\newcommand{\tosquare}{\stackrel{L^2}{\to}}
\newcommand{\bsl}{\backslash}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bu}{\mathbf{u}}


\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bEta}{\boldsymbol{\eta}}
\newcommand{\dd}{{\,\rm d}}

\newcommand{\stirling}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
\newcommand{\stirlingsec}[2]{\genfrac{\{}{\}}{0pt}{}{#1}{#2}}

\newcommand{\given}{\,|\,}
\newcommand{\bgiven}{\,\big|\,}



==> facts.tex <==
\section{Auxiliary results}\label{facts}

\subsection{Blaschke-Petkantschin type formulae}

% The following result (\cite{SW08}, Theorem 7.2.7) is widely used when dealing with convex hulls of random points in a given convex body:

% \begin{st}[Blaschke-Petkantschin formula]\label{BPf}
% Let $h:(\mathbb{R}^d)^{l+1} \rightarrow \mathbb R$ be non-negative measurable function, $l~\in \left\{1, . . . , d \right\}$. Then 
% \begin{align*}
%     &\int\limits_{(\mathbb{R}^d)^{l+1}}{f(x_0, \ldots , x_l) \mathrm{d}x_0 \ldots \mathrm{d}x_l} = \\ \notag
%     &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}{\int\limits_{E^{l+1}}{f(x_0, \ldots , x_l){|\mathrm{conv}(x_0, \ldots, x_l)|}^{d-l}\lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E)},
% \end{align*}
% where $b_{d,k} = \frac{\omega_{d-k+1} \cdots \omega_{d}}{\omega_1 \cdots \omega_k}$.
% \end{st}


% To prove Theorem \ref{thm1}  we are going to need the analogous formula for points distributed on the boundary of the convex body (\cite{Zahle}, \cite{Reitzner}):

% \begin{st}[Z\"ahle formula]\label{Zahlest}
% Let $X$ be a $(d-1)$-dimensional measurable set and let $g(x_0,\ldots, x_l)$ be a measurable function, $l\leq d$. Then 

% \begin{align*}
%     &\int\limits_{A_{d,l}}{\int\limits_{(E\cap  X)^{l+1}}g(x_0, \ldots , x_l) \mathbbm{1}_{\{x_0, \ldots, x_l \;\text{ in general position}\}} \sigma_{E\cap X}(\mathrm{d}x_0)\ldots \sigma_{E\cap X}(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E) = \\
%     &= \frac{1}{(l!)^{d-l}b_{d,l}}
%     \int\limits_{X^{l+1}} g(x_0, \ldots , x_l) \mathbbm{1}_{\{x_0, \ldots, x_l\; \text{ in general position}\}} \frac{1}{|\mathrm{conv}(x_0, \ldots, x_l)|^{d-l}} \times \\ 
%     &\times\prod_{k=0}^{l}\|P_E(n_X(x_k))\| \sigma_{X}(\mathrm{d}x_0) \ldots \sigma_{X}(\mathrm{d}x_l).
% \end{align*}

% where $n_X(P)$ denotes the outer unit normal vector of $X$ at $P$ and $P_E$ is the orthogonal projection onto the hyperplane $E$.

% \end{st}

\begin{cor}
Consider the case of $l=1, X = \partial K$, $K$ -- convex body with smooth boundary. In this case we have a random line $g$ intersecting $\partial K$ at points $P_1$ and $P_2$. Then Z\"ahle formula can be rewritten the following way:

\begin{align}\label{eq:zahle2p}
    \int\limits_{A_{d,1}} g(P_1,P_2) \mu_{d,1}(\mathrm{d}g) = \frac{1}{\omega_d}\int\limits_{(\partial K)^2} g(P_1,P_2)\frac{\sin\alpha_1\sin\alpha_2}{|\chi(P_1,P_2)|^{d-1}} \sigma(\mathrm{d}P_1)\sigma(\mathrm{d}P_2),
\end{align}

where $\alpha_1$ and $\alpha_2$ are the angles between line $P_1P_2$ and tangent hyperplanes at points $P_1$ and $P_2$.

\end{cor}

\begin{cor}
Consider the case $X = \partial P$, where $P$ is a convex polytope.
In this case $\|P_E(n_X(x_k))\| = 0$ if and only if all points $x_k$ lie on the same facet of $P$. 
Then for measurable function $g$ we have 

\begin{align*}
    &\int\limits_{(\partial P)^{l+1}} g(x_0,\ldots, x_l) \sigma_{\partial P}(\mathrm{d}x_0) \ldots \sigma_{\partial P}(\mathrm{d}x_l) = \\
    &= \int\limits_{(\partial P)^{l+1}} g(x_0, \ldots, x_l)\mathbbm{1}_{\{x_1, \ldots, x_l \,\text{are not all in the same facet}\}} \sigma_{\partial P}(\mathrm{d}x_0) \ldots \sigma_{\partial P}(\mathrm{d}x_l) + \\
    &+ \sum_{F - \text{ facet of}\, P} \int\limits_{F^{l+1}} g(x_0,\ldots, x_l) \lambda_F(\mathrm{d}x_0) \ldots \lambda_F(\mathrm{d}x_l). 
\end{align*}
Applying Statement~\ref{Zahlest} to the first term and Statement~\ref{BPf} to the second term we get the following:

\begin{align*}
     \int\limits_{(\partial P)^{l+1}} g(x_0,&\ldots, x_l) \sigma_{\partial P}(\mathrm{d}x_0) \ldots \sigma_{\partial P}(\mathrm{d}x_l) = \\
    & = (l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}
    \int\limits_{(E\cap  \partial P)^{l+1}} g(x_0, \ldots, x_l)
     \mathbbm{1}_{\{x_1, \ldots, x_l \,\text{are not all in the same facet}\}} \times \\
     &\times |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l} 
    \prod_{k=0}^{l}\|P_E(n_P(x_k))\|^{-1} 
     \sigma_{E\cap \partial P}(\mathrm{d}x_0)\ldots 
     \sigma_{E\cap \partial P}(\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E) + \\
     &+ (l!)^{d-l-1}b_{d-1,l}\cdot \sum_{F - \text{facet of}\, P} 
     \int\limits_{A_{d-1,l}}\int\limits_{(H \cap F)^{l+1}} g(x_0, \ldots, x_l) \times \\
     &\times 
     |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l-1}\lambda_{H \cap F}(\mathrm{d}x_0)\ldots \lambda_{H \cap F}(\mathrm{d}x_l)\mu_{d-1,l}(\mathrm{d}E) = \\
     &= (l!)^{d-l}b_{d,l} 
     \sum_{(F_0, \ldots, F_l) - \text{facets of }P, \text{ not all the same}}
     \int\limits_{A_{d,l}}\int\limits_{E\cap F_0}\ldots
     \int\limits_{E\cap F_l} g(x_0, \ldots, x_l) \times \\
     &\times
     |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l} \prod_{k=0}^{l}\|P_E(n_P(x_k))\|^{-1} \lambda_{E \cap F_0 }(\mathrm{d}x_0)\ldots \lambda_{E \cap F_l}
     (\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E) + \\
     &+ (l!)^{d-l-1}b_{d-1,l}\cdot \sum_{F - \text{facet of}\, P} 
     \int\limits_{A_{d-1,l}}\int\limits_{(H \cap F)^{l+1}} g(x_0, \ldots, x_l) \times \\
     &\times 
     |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l-1}\lambda_{H\cap F}(\mathrm{d}x_0)\ldots \lambda_{H \cap F}(\mathrm{d}x_l)\mu_{d-1,l}(\mathrm{d}E). 
\end{align*}

\end{cor}

\bigskip

% In section \ref{NewZahle} we are going to prove the following generalisation of Z\"ahle formula for convex bodies with smooth boundary:

% \begin{thm}\label{thm3}

%     Let $K$ be a convex body with smooth boundary and let $g(x_0,\ldots, x_l)$ be a continuous function, $l\leq d, k \leq l+1$. Then 
    
% \begin{align*}
%      &\int\limits_{(\partial K)^{k}}\int\limits_{(K)^{l-k+1}}g(x_0, \ldots , x_l) \mathrm{d}x_{0} \ldots \mathrm{d}x_{l-k} 
%      \sigma_{\partial K}(\mathrm{d}x_{l-k+1}) \ldots 
%      \sigma_{\partial K}(\mathrm{d}x_l) = \\ 
%     &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}
%     \int\limits_{(E\cap \partial K)^{k}}
%     \int\limits_{(E \cap K)^{l-k+1}}g(x_0, \ldots , x_l)
%     {|\mathrm{conv}(x_0, \ldots, x_l)|}^{d-l}\times \\
%     &\times \prod_{j=l-k+1}^{l}\|P_E(n_K(x_k))\|^{-1} \lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_l-k) 
%     \sigma_{E\cap \partial K}(\mathrm{d}x_{l-k+1})\ldots 
%     \sigma_{E\cap \partial K}(\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E),
% \end{align*}

% where $n_K(P)$ denotes the outer unit normal vector of $K$ at $P$ and $P_E$ is the orthogonal projection onto the hyperplane $E$.

% \end{thm}


\subsection{Flag spaces}

Let $p, q \in \{0, \ldots, d\}$, and let $E \in A(d, p)$ be a fixed $p$-dimensional affine subspace. Denote by $A(L, q)$ the space of all $q$-dimensional affine subspaces
contained in $E$ if $q \leqslant p$, respectively containing $E$ if $q \geqslant p$. By $\mu_E^q$ denote invariant measure on $A(E, q)$  (\cite{SW08}, Section 7.1). 

Consider pairs of affine subspaces:
\begin{align*}
    &A(d, p, q) := \{(E,F) \in A(d, p) \times A(d, q) : E \subset F\},\; \text{if}\; p < q, \\
&A(d, p, q) := \{(E,F) \in A(d, p) \times A(d, q) : E \supset F\},\; \text{if}\; p > q.
\end{align*}

We are going to need the following result:

\begin{st}
If $0 \leqslant p < q \leqslant d-1$ and $f : A(d, p, q) \rightarrow \mathbb{R}$ is a nonnegative measurable function, then

\begin{align}\label{eq:flags}
    &\int\limits_{A(d,q)}\int\limits_{A_{F,p}} f(E,F)\mu_p^F(\mathrm{d}E)\mu_{d,q}(\mathrm{d}F) = 
     \int\limits_{A(d,p)}\int\limits_{A_{E,q}} f(E,F)\mu_q^E(\mathrm{d}F)\mu_{d,p}(\mathrm{d}E).
\end{align}

\end{st}

==> intro_rus.tex <==
\section{Введение}

Рассмотрим выпуклое тело $K$ в $\R^d$ и обозначим за $|K|$ его объем ($d$-мерную меру Лебега). Обозначим за $\partial K$ границу $K$, снабженную $(d-1)$-мерной мерой Хаусдорфа $\sigma_{\partial K}$. Для краткости мы будем использовать обозначение $\sigma$ вместо $\sigma_{\partial K}$ в случаях, когда из контекста ясно, граница какого тела рассматривается %не вводит в заблуждение? уместно?
Также для краткости мы будем использовать обозначение $|\partial K|=\sigma(\partial K)$. 

% For a convex body $K$ in $\R^d$ denote by $|K|$ its volume (the $d$-dimensional Lebesgue measure). Denote by $\partial K$ the boundary of $K$ equipped with the $(d-1)$-dimensional Haisdorff measure $\sigma_{\partial K}$.  When it causes no confusion, for abbreviation we use just $\sigma$ instead of $\sigma_{\partial K}$. Also for simplicity we write $|\partial K|=\sigma(\partial K)$. 

Пусть $l \in \{1, \ldots, d\}$. Обозначим за $A_{d,l}$ множество всех аффиных $l$-мерных плоскостей в $\R^d$ с мерой Хаара $\mu_{d,l}$, инвариантной относительно поворотов и параллельных переносов и нормированной следующим образом:

\begin{align}\label{2104_rus}
    \mu_{d,l}\left(\left\{E\in A_{d,l}:\,E\cap \B^d\ne\emptyset\right\}\right)=\kappa_{d-l},
\end{align}

где $\B^k$ есть $k$-мерный едичиный шар, а $\kappa_k:=|\mathbb B^k|$. Обозначим также $\omega_k:=|\mathbb{S}^{k-1}|=k\kappa_k$, где $\mathbb{S}^{k-1}=\partial \B^k$ --- $(k-1)$-мерная едичиная сфера. 

% For $l \in \{1, \ldots, d\}$ denote by $A_{d,l}$ the set of all affine $l$-planes in $\R^d$ equipped with the unique Haar measure $\mu_{d,l}$ invariant with respect to the rigid motions and normalized by
% \begin{align}\label{2104}
%     \mu_{d,l}\left(\left\{E\in A_{d,l}:\,E\cap \B^d\ne\emptyset\right\}\right)=\kappa_{d-l},
% \end{align}
% where $\B^k$ is  the $k$-dimensional unit ball and $\kappa_k:=|\mathbb B^k|$. Also let $\omega_k:=|\mathbb{S}^{k-1}|=k\kappa_k$, where $\mathbb{S}^{k-1}=\partial \B^k$ is the $(k-1)$-dimensional unit sphere.

Для конечного множества точек $x_1,\dots,x_n$ в $\R^d$ обозначим за $[x_1,\dots,x_n]$ их выпуклую оболочку. В частности, $[x_1,x_2]$ обозначает отрезок с концами в точках $x_1$ и $x_2$.

% Given a finite number of points $x_1,\dots,x_n\in\R^d$ denote by $[x_1,\dots,x_n]$ their convex hull. In particular, $[x_1,x_2]$ is
% the segment with endpoints $x_1$ and $x_2$.


\bigskip

Рассмотрим случай $d=2$. 
Пусть $K$ --- выпуклая фигура на плоскости с $C^1$-гладкой границей. Рассмотрим случайную прямую $G$, пересекающую $K$, выбранную в соответствии с мерой Хаара $\mu_{2,1}$.

% We start with the case $d=2$.
% Let $K$ be a planar convex body with $C^1$ boundary. Consider a random line $G$ intersecting $K$ chosen with respect to the measure $\mu_{2,1}$.

В \cite{Pleijel} Плейелем было получено тождество, позволяющее выразить среднее значение $h(|G \cap K|)$ в терминах интегрирования по границе $K$ для всех функций $h$, имеющих непрерывную производную и таких, что $h(0)=0$:
\begin{align}\label{eq:pleijel_rus}
    \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{2,1}(\dd G)  \\ \notag
    &= \frac{1}{2}\int\limits_{(\partial K)^2} h'(|x_1 - x_2|)\cos\alpha_1\cos\alpha_2\, \sigma(\dd x_1)\sigma(\dd x_2),
\end{align}
где   $\alpha_1$ и $\alpha_2$ --- углы между касательными в точках $x_1$ и  $x_2$ и хордой $[x_1,x_2]$, лежащие по одну сторону от хорды.
Кроме того, Плейель показал, что 
\begin{align}\label{eq:pleijelcot_rus}
    \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{2,1}(\dd G)  \\ \notag 
    &= \int\limits_{G \cap K \neq \emptyset} h'(|G \cap K|)|G \cap K|\cot\alpha_1\cot\alpha_2 \mu_{2,1}(\dd G).
\end{align}

Из равенства \eqref{eq:pleijel_rus} можно вывести (см.\cite[Раздел 6.9]{AMS89}) явную форму дефекта в изопериметрическом неравенстве: 
\begin{align*}%\label{defect}
    |\partial K|^2 - 4\pi |K| = 2\int\limits_{(\partial K)^2} \sin^2\frac{\alpha_1 - \alpha_2}{2} \sigma(\dd x_1)\sigma(\dd x_2). 
\end{align*}


% In \cite{Pleijel} Pleijel discovered an identity
% expressing the expectation of $h(|G \cap K|)$ in terms of the intergation over the boundary of $K$ for all functions $h$ with continuous derivative and such that $h(0)=0$:
% \begin{align}\label{eq:pleijel}
%     \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{2,1}(\dd G)  \\ \notag
%     &= \frac{1}{2}\int\limits_{(\partial K)^2} h'(|x_1 - x_2|)\cos\alpha_1\cos\alpha_2\, \sigma(\dd x_1)\sigma(\dd x_2),
% \end{align}
% where  $\alpha_1$ and $\alpha_2$ are angles between tangents at points $x_1$ and $x_2$
% and the chord  $[x_1,x_2]$. Here we consider the  tangents 
% lying on the same side of the chord. Moreover, Pleijel showed that
% \begin{align}\label{eq:pleijelcot}
%     \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{2,1}(\dd G)  \\ \notag 
%     &= \int\limits_{G \cap K \neq \emptyset} h'(|G \cap K|)|G \cap K|\cot\alpha_1\cot\alpha_2 \mu_{2,1}(\dd G).
% \end{align}
% From~\eqref{eq:pleijel} it is possible to derive \textcolor{red}{(see, e.g., \cite[???]{AMS89})} an explicit form of the defect in the isoperimetric inequality:
% \begin{align*}%\label{defect}
%     |\partial K|^2 - 4\pi |K| = 2\int\limits_{(\partial K)^2} \sin^2\frac{\alpha_1 - \alpha_2}{2} \sigma(\dd x_1)\sigma(\dd x_2). 
% \end{align*}

Абмарцумяном в \cite{AMB} было получено комбинаторное доказательство тождества Плейеля а также представлена его версия для выпуклых плоских многоугольников, также известная как тождество Амбарцумяна-Плейеля: пусть $P$ --- выпуклый многоугольник с длинами сторон $a_1, \ldots, a_n$, тогда 
\begin{align}\label{eq:ambpleijelcot_rus}
    &\int\limits_{G \cap P \neq \emptyset} h(|G \cap P|) \mu_{2,1}(\dd G) \\ \notag 
    &= \int\limits_{G \cap P \neq \emptyset} h'(|G \cap P|)|G \cap P|\cot\alpha_1\cot\alpha_2 \mu_{2,1}(\dd G) + \sum_{i = 1}^n \int\limits_{0}^{a_i} h(t) \mathrm{d}t.
\end{align}

% In \cite{AMB}, Ambartzumian gave a combinatorial proof of the Pleijel identity and presented  its version  for the convex planar polygons which is now known as the Ambartzumian--Pleijel identity: if $P$ is a convex polygon with side lengths $a_1, \ldots, a_n$, then 
% \begin{align}\label{eq:ambpleijelcot}
%     &\int\limits_{G \cap P \neq \emptyset} h(|G \cap P|) \mu_{2,1}(\dd G) \\ \notag 
%     &= \int\limits_{G \cap P \neq \emptyset} h'(|G \cap P|)|G \cap P|\cot\alpha_1\cot\alpha_2 \mu_{2,1}(\dd G) + \sum_{i = 1}^n \int\limits_{0}^{a_i} h(t) \mathrm{d}t.
% \end{align}

Существует аналог тождества Плейеля для выпуклых тел с гладкой границей в $\R^3$ (см. \cite{AMB82}): 
\begin{align*}%\label{pleijel3}
    \int\limits_{G \cap K \neq \emptyset}& h(|G \cap K|) \mu_{3,1}(\dd G)  \\ \notag 
    &= 4\int\limits_{(\partial K)^2} \frac{h'(|x_1 - x_2|)}{|x_1 - x_2|}\cos\alpha_1\cos\alpha_2\cos\phi_0 \sigma(\dd x_1)\sigma(\dd x_2),
\end{align*} 
где $\alpha_1, \alpha_2$ --- углы между хордой $[x_1,x_2]$ и ее проекциями на касательные плоскости, а $\phi_0$ --- угол между проекциями нормалей в точках $x_1$, $x_2$ на ортогональное дополнение прямой, прододящей через точки $x_1$ и $x_2$. 


% There exists an analogue of the Pleijel identity for the convex bodies with  smooth boundary in $\R^3$, see \cite{AMB82}:
% \begin{align*}%\label{pleijel3}
%     \int\limits_{G \cap K \neq \emptyset}& h(|G \cap K|) \mu_{3,1}(\dd G)  \\ \notag 
%     &= 4\int\limits_{(\partial K)^2} \frac{h'(|x_1 - x_2|)}{|x_1 - x_2|}\cos\alpha_1\cos\alpha_2\cos\phi_0 \sigma(\dd x_1)\sigma(\dd x_2),
% \end{align*}
% where $\alpha_1, \alpha_2$ are the angles between the chord $[x_1,x_2]$ and its projections onto the tangent planes, and $\phi_0$ is the angle between projections of normal vectors at points $x_1$ and $x_2$ onto the orthogonal complement of the line passing through the points $x_1,x_2$.

Первый результат данной статьи --- обобщение тождества Плейеля на случай произвольной размерности. 
\begin{thm}\label{thm1_rus}
Рассмотрим выпуклое тело $K$ в $\mathbb{R}^d$ с $C^1$-гладкой границей. Для любой функции  $h: \mathbb{R} \rightarrow \mathbb{R}$, имеющей непрерывную производную и такой, что $h(0)=0$, имеем:
\begin{align*}%\label{orbdim}
    \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{d,1}(\dd G) \\ \notag  
    &= \frac{1}{(d-1)\omega_d}\int\limits_{(\partial K)^2} \frac{h'(|x_1 - x_2|)}{|x_1 - x_2|^{d-2}}\cos\alpha_1\cos\alpha_2\cos\phi_0 \sigma(\dd x_1)\sigma(\dd x_2),
\end{align*}
где  $\alpha_1,\alpha_2$ --- углы между хордой $[x_1,x_2]$  и ее проекциями на касательные плоскости, а $\phi_0$ --- угол между проекциями нормалей в точках $x_1$, $x_2$ на ортогональное дополнение прямой, проходящей через $x_1$ и $x_2$.
\end{thm}

% Our first result is the following generalization of the Pleijel identity to arbitrary dimension.
% \begin{thm}\label{thm1}
% Let K be a convex body in $\mathbb{R}^d$ with $C^1$ boundary. Then for every function $h: \mathbb{R} \rightarrow \mathbb{R}$ with continuous derivative such that $h(0)=0$ we have
% \begin{align*}%\label{orbdim}
%     \int\limits_{G \cap K \neq \emptyset} &h(|G \cap K|) \mu_{d,1}(\dd G) \\ \notag  
%     &= \frac{1}{(d-2)\omega_d}\int\limits_{(\partial K)^2} \frac{h'(|x_1 - x_2|)}{|x_1 - x_2|^{d-2}}\cos\alpha_1\cos\alpha_2\cos\phi_0 \sigma(\dd x_1)\sigma(\dd x_2),
% \end{align*}
% where  $\alpha_1,\alpha_2$ are the angles between the chord $[x_1,x_2]$  and its projections onto the tangent planes, and $\phi_0$ is the angle between projections of normal vectors at points $x_1$ and $x_2$ onto the orthogonal complement of the line passing through the points $x_1,x_2$.
% \end{thm}

Для того, чтобы сформулировать дальнейшие результаты, нам понадобится ввести некоторые обозначения для подмножеств меньшей размерности. Для некоторых $E\in A_{d,l}$  и $k\in\{1,\dots,l\}$ обозначим за $A_{E,k}$ множество всех аффинных $k$-мерных плоскостей в $E\cong\R^l$, снабженное мерой Хаара $\mu_{E,k}$, инвариантной относительно движений и нормированной так же, как в~\eqref{2104_rus}. Для произвольного подмножества $M\subset\R^d$ обозначим 
\begin{align*}
    A_{M,k}=A_{\mathrm{aff}M,k}, \quad \mu_{M,k}=\mu_{\mathrm{aff}M,k},
\end{align*}
где $\mathrm{aff}M$ есть аффинная оболочка $M$ --- пересечение всех аффинных плоскостей, содержащих $M$. Обозначим также за $\lambda_E$ $l$-мерную меру Лебега на $E$. 

% To formulate our further results, we need to extend some of our notation to subsets of lower dimension. Given some $E\in A_{d,l}$ and $k\in\{1,\dots,l\}$ denote by $A_{E,k}$ the set of all affine $k$-planes in $E\cong\R^l$ equipped with the unique Haar measure $\mu_{E,k}$ invariant with respect to the rigid motions and normalized the same way as in~\eqref{2104}. Now for an arbitrary subset $M\subset\R^d$ we write
% \begin{align*}
%     A_{M,k}=A_{\mathrm{aff}M,k}, \quad \mu_{M,k}=\mu_{\mathrm{aff}M,k},
% \end{align*}
% where $\mathrm{aff}M$ denotes the affine span of $M$, the intersection of all affine planes containing $M$. We also denote by $\lambda_E$ the $l$-dimensional Lebesgue measure in $E$.

Следующий результат данной работы обощает тождество Амбарцумяна-Плейеля (\eqref{eq:ambpleijelcot_rus}) на случай произвольной размерности. Для выпуклого многогранника $P$ обозначим за $\mathcal F(P)$ множество его гиперграней. 
\begin{thm}\label{thm2_rus}
    Пусть $P$ --- выпуклый многогранник в $\mathbb{R}^d$. Тогда для любой функции $h: \mathbb{R} \rightarrow \mathbb{R}$, имеющей непрерывную производную и такой, что $h(0)=0$, выполнено
\begin{align*}
    \int\limits_{G \cap P \neq \emptyset} &h(|G \cap P|) \mu_{d,1}(\dd G) = \frac{1}{(d-1)}\int\limits_{G \cap P \neq \emptyset} h'(|G \cap P|)|G \cap P|\cot\alpha_1\cot\alpha_2\cos\phi_0 \mu_{d,1}(\dd G)  \\ \notag &+ \sum_{F\in\mathcal F(P)} \int\limits_{A_{F,1}} H(|G \cap F|) \mu_{F,1}(\mathrm{d}G),
\end{align*}
где $\alpha_1,\alpha_2$ --- углы между хордой $G \cap P$ и ее проекциями на касательные гиперплоскости,  $\phi_0$ --- угол между проекциями нормалей в концах $G \cap P$ на орторональное дополнение прямой  $G$, а $H$ --- первообразная $h$. 
\end{thm}


% Our next result generalizes the Ambartzumian--Pleijel identity (see~\eqref{eq:ambpleijelcot}) to higher dimensions. Given a convex polytope $P$ denote by $\mathcal F(P)$ the set of its facets.
% \begin{thm}\label{thm2}
% Let P be a convex polytope in $\mathbb{R}^d$. Then for every function $h: \mathbb{R} \rightarrow \mathbb{R}$ with continuous derivative such that $h(0)=0$ we have
% \begin{align*}
%     \int\limits_{G \cap P \neq \emptyset} &h(|G \cap P|) \mu_{d,1}(\dd G) = \frac{1}{(d-2)}\int\limits_{G \cap P \neq \emptyset} h'(|G \cap P|)|G \cap P|\cot\alpha_1\cot\alpha_2\cos\phi_0 \mu_{d,1}(\dd G)  \\ \notag &+ \sum_{F\in\mathcal F(P)} \int\limits_{A_{F,1}} H(|G \cap F|) \mu_{F,1}(\mathrm{d}G),
% \end{align*}
% where $\alpha_1,\alpha_2$ are the angles between the chord $G \cap P$ and its projections onto the tangent planes,  $\phi_0$ is the angle between projections of normal vectors at endpoints of $G \cap P$ onto the orthogonal complement of line $G$, and $H$ is the antiderivative of $h$. 
% \end{thm}

Сформулированная ниже формула Бляшке-Петканчина (\cite{SW08}, Теорема 7.2.7) широко используется при работе с выпуклыми оболочками точек, случайно выбранных внутри данного выпуклого тела:
пусть $h:(\mathbb{R}^d)^{l+1} \rightarrow \mathbb R$ --- измеримая функция, $l~\in \left\{1, . . . , d \right\}$, тогда 
\begin{align}\label{BPF_rus}
    &\int\limits_{(\mathbb{R}^d)^{l+1}}{h(x_0, \ldots , x_l) \mathrm{d}x_0 \ldots \mathrm{d}x_l}  \\ \notag
    &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}{\int\limits_{E^{l+1}}{h(x_0, \ldots , x_l){|[x_0, \ldots, x_l]|}^{d-l}\lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E)},
\end{align}
где  $b_{d,k} = \frac{\omega_{d-k+1} \cdots \omega_{d}}{\omega_1 \cdots \omega_k}$.

% The following Blaschke--Petkantschin formula  (see, e.g.,~\cite{SW08}, Theorem 7.2.7) is widely used when dealing with the convex hulls of random points in a given convex body:
% if $h:(\mathbb{R}^d)^{l+1} \rightarrow \mathbb R$ is а non-negative  measurable function, $l~\in \left\{1, . . . , d \right\}$, then 
% \begin{align}\label{BPF}
%     &\int\limits_{(\mathbb{R}^d)^{l+1}}{h(x_0, \ldots , x_l) \mathrm{d}x_0 \ldots \mathrm{d}x_l}  \\ \notag
%     &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}{\int\limits_{E^{l+1}}{h(x_0, \ldots , x_l){|\mathrm{conv}(x_0, \ldots, x_l)|}^{d-l}\lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E)},
% \end{align}
% where $b_{d,k} = \frac{\omega_{d-k+1} \cdots \omega_{d}}{\omega_1 \cdots \omega_k}$.

Для доказательства Теоремы \ref{thm1} нам понадобится формула Цэле, являющаяся аналогом формулы Бляшке-Петканчина в случае, когда точки случайно выбираются на границе выпуклого тела (\cite{Zahle}, \cite{Reitzner}):
пусть $K$ --- выпуклое тело в $\R^d$,  $h:(\mathbb{R}^d)^{l+1} \rightarrow \mathbb R$ --- измеримая функция, $l\leq d$, тогда
\begin{align}\label{Zahle_rus}
    &\int\limits_{A_{d,l}}{\int\limits_{(E\cap  \partial K)^{l+1}}h(x_0, \ldots , x_l) 
    \mathbbm{1}_{\{x_0, \ldots, x_l \;\text{ in general position}\}} \sigma_{E\cap \partial K}(\mathrm{d}x_0)\ldots \sigma_{E\cap \partial K}(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E) \\ \notag
    &= \frac{1}{(l!)^{d-l}b_{d,l}}
    \int\limits_{(\partial K)^{l+1}} h(x_0, \ldots , x_l) \mathbbm{1}_{\{x_0, \ldots, x_l\; \text{ in general position}\}} \frac{1}{|[x_0, \ldots, x_l]|^{d-l}}  \\ \notag
    &\times\prod_{k=0}^{l}\|\mathrm{P}_{\mathrm{aff}(x_0, \ldots, x_l)}(n_K(x_k))\| 
    \sigma_{\partial K}(\mathrm{d}x_0) \ldots \sigma_{\partial K}(\mathrm{d}x_l),
\end{align}
где  $n_K(x)$ обозначает внешнюю нормаль к $\partial K$ в точке $x$, а 
$\mathrm{P}_E$ есть ортогональная проекция на плоскость $E$. 


% To prove Theorem \ref{thm1}  we will need the following Z\"ahle formula which is a counterpart of the  Blaschke--Petkantschin formula for points distributed over the boundary of the convex body (\cite{Zahle}, \cite{Reitzner}):
% if $K$ is a convex body in $\R^d$ and $h:(\mathbb{R}^d)^{l+1} \rightarrow \mathbb R$ is a measurable function, $l\leq d$, then 
% \begin{align}\label{Zahle}
%     &\int\limits_{A_{d,l}}{\int\limits_{(E\cap  \partial K)^{l+1}}h(x_0, \ldots , x_l) 
%     \mathbbm{1}_{\{x_0, \ldots, x_l \;\text{ in general position}\}} \sigma_{E\cap \partial K}(\mathrm{d}x_0)\ldots \sigma_{E\cap \partial K}(\mathrm{d}x_l)}\mu_{d,l}(\mathrm{d}E) \\ \notag
%     &= \frac{1}{(l!)^{d-l}b_{d,l}}
%     \int\limits_{(\partial K)^{l+1}} h(x_0, \ldots , x_l) \mathbbm{1}_{\{x_0, \ldots, x_l\; \text{ in general position}\}} \frac{1}{|\mathrm{conv}(x_0, \ldots, x_l)|^{d-l}}  \\ \notag
%     &\times\prod_{k=0}^{l}\|P_E(n_K(x_k))\| 
%     \sigma_{\partial K}(\mathrm{d}x_0) \ldots \sigma_{\partial K}(\mathrm{d}x_l),
% \end{align}
% where $n_K(x)$ denotes the outer unit normal vector of $\partial K$ at $x$ and $P_E$ is the orthogonal projection onto the hyperplane $E$.

\bigskip

В работе мы приводим следующее обобщение одновременно формул Бляшке-Петканчина и Цэле для выпуклых тел с гладкой границей:

\begin{thm}\label{thm3_rus}

    Пусть $K$ --- выпуклое тело в $\R^d$ с гладкой границей,  $h(x_0,\ldots, x_l)$ --- непрерывная функция, $l\leq d$. Тогда для всех $k\in\{0,\dots, l+1\}$  имеем
\begin{align*}
     &\int\limits_{(\partial K)^{k}}\int\limits_{(K)^{l-k+1}}h(x_0, \ldots , x_l) \mathrm{d}x_{0} \ldots \mathrm{d}x_{l-k} 
     \sigma_{\partial K}(\mathrm{d}x_{l-k+1}) \ldots 
     \sigma_{\partial K}(\mathrm{d}x_l)  \\ 
    &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}
    \int\limits_{(E\cap \partial K)^{k}}
    \int\limits_{(E \cap K)^{l-k+1}}h(x_0, \ldots , x_l)
    {|[(x_0, \ldots, x_l]|}^{d-l} \\
    &\times \prod_{j=l-k+1}^{l}\|\mathrm{P}_E(n_K(x_k))\|^{-1} \lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_{l-k}) 
    \sigma_{E\cap \partial K}(\mathrm{d}x_{l-k+1})\ldots 
    \sigma_{E\cap \partial K}(\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E),
\end{align*}
где  $n_K(x)$ обозначает внешнюю нормаль к $K$ в точке $x$, а $\mathrm{P}_E$ есть ортогональная проекция на плоскость $E$.

\end{thm}

% In this paper we  prove the following generalisation of both the Blaschke-Petkantschin and the Z\"ahle formulae for convex bodies with smooth boundary:

% \begin{thm}\label{thm3}

%     Let $K$ be a convex body with smooth boundary and let $h(x_0,\ldots, x_l)$ be a continuous function, $l\leq d$. Then for all $k\in\{0,\dots, l+1\}$ we have
% \begin{align*}
%      &\int\limits_{(\partial K)^{k}}\int\limits_{(K)^{l-k+1}}h(x_0, \ldots , x_l) \mathrm{d}x_{0} \ldots \mathrm{d}x_{l-k} 
%      \sigma_{\partial K}(\mathrm{d}x_{l-k+1}) \ldots 
%      \sigma_{\partial K}(\mathrm{d}x_l)  \\ 
%     &=(l!)^{d-l}b_{d,l}\int\limits_{A_{d,l}}
%     \int\limits_{(E\cap \partial K)^{k}}
%     \int\limits_{(E \cap K)^{l-k+1}}h(x_0, \ldots , x_l)
%     {|\mathrm{conv}(x_0, \ldots, x_l)|}^{d-l} \\
%     &\times \prod_{j=l-k+1}^{l}\|P_E(n_K(x_k))\|^{-1} \lambda_{E}(\mathrm{d}x_0)\ldots \lambda_E(\mathrm{d}x_{l-k}) 
%     \sigma_{E\cap \partial K}(\mathrm{d}x_{l-k+1})\ldots 
%     \sigma_{E\cap \partial K}(\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E),
% \end{align*}
% where $n_K(x)$ denotes the outer unit normal vector of $K$ at $x$ and $P_E$ is the orthogonal projection onto the hyperplane $E$.

% \end{thm}

Рассмотрим случай $k=l=1$, когда одна точка выбирается на границе тела, а одна внутри. 
Применяя Теорему~\ref{thm3_rus} к функции $h(x_0, x_1) = |x_0 - x_1|^n$ для некоторого целого $n$, получаем аналог формулы Кингмана \cite{jK69}, которая утверждает, что $n$-й момент расстояния между точками, случайно выбранными внутри выпуклого тела, с точностью до некоторой константы совпадает с $(n+d+1)$-м моментом длины случайной хорды. 
\begin{corollary}
Для выпуклого тела $K$ с гладкой границей имеем
\[
     \int\limits_{\partial K}\int\limits_{K} |x_0 - x_1|^n \mathrm{d}x_{0} \sigma_{\partial K}(\mathrm{d}x_{1}) = \frac{\omega_d}{4}\int\limits_{A_{d,1}} \frac{|G \cap K|^{n+d}}{n+d}\left(\frac{1}{\sin \alpha_1} + \frac{1}{\sin \alpha_2}\right)\mu_{d,1}(\mathrm{d}G).
\]
\end{corollary}
\begin{proof}
Применяя Теорему~\ref{thm3_rus} к функции $h(x_0, x_1) = |x_0 - x_1|^n$, получаем
\begin{align*}
    \int\limits_{\partial K}\int\limits_{K} &|x_0 - x_1|^n \mathrm{d}x_{0} \sigma_{\partial K}(\mathrm{d}x_{1})    \\
    &=
    \frac{\omega_{d}}{4} \int\limits_{A_{d,1}}  \left(\frac{1}{\sin \alpha_1}\int\limits_{G\cap K}|x_0 - x_1|^{n+d-1} \lambda_G(\mathrm{d}x_0) + \frac{1}{\sin \alpha_2}\int\limits_{G\cap K}|x_0 - x_2|^{n+d-1} \lambda_G(\mathrm{d}x_0) \right)\mu_{d,1}(\mathrm{d}G),
\end{align*}
где $\alpha_i$ --- угол между прямой $G$ и касательной гиперплоскостью в точке $x_i$. Используя
\[
    \int\limits_{G \cap K} |x_0 - x_i|^{n+d-1} \lambda_G(\mathrm{d}x_0) = \int\limits_0^{|G \cap K|} x^{n+d-1} \mathrm{d}x = \frac{|G \cap K|^{n+d}}{n+d}
\]
мы получаем требуемое.
\end{proof}
    
% Consider the case $k=l=1$, i.e. we have one point on the boundary and one point inside $K$. 
% Applying Theorem~\ref{thm3} to the function $h(x_0, x_1) = |x_0 - x_1|^n$ for some integer $n$ implies a counterpart of Kingman's formula \cite{jK69}, which states that the $n$-th moment of the distance between two points randomly chosen inside the body is up to some constant equal to the $(n+d+1)$-st moment of the length of random chord
% \begin{corollary}
% For a convex body $K$ with smooth boundary we have
% \[
%      \int\limits_{\partial K}\int\limits_{K} |x_0 - x_1|^n \mathrm{d}x_{0} \sigma_{\partial K}(\mathrm{d}x_{1}) = \frac{\omega_d}{4}\int\limits_{A_{d,1}} \frac{|G \cap K|^{n+d}}{n+d}\left(\frac{1}{\sin \alpha_1} + \frac{1}{\sin \alpha_2}\right)\mu_{d,1}(\mathrm{d}G).
% \]
% \end{corollary}
% \begin{proof}
% Applying Theorem~\ref{thm3} with $h(x_0, x_1) = |x_0 - x_1|^n$ gives
% \begin{align*}
%     \int\limits_{\partial K}\int\limits_{K} &|x_0 - x_1|^n \mathrm{d}x_{0} \sigma_{\partial K}(\mathrm{d}x_{1})    \\
%     &=
%     \frac{\omega_{d}}{4} \int\limits_{A_{d,1}}  \left(\frac{1}{\sin \alpha_1}\int\limits_{G\cap K}|x_0 - x_1|^{n+d-1} \lambda_G(\mathrm{d}x_0) + \frac{1}{\sin \alpha_2}\int\limits_{G\cap K}|x_0 - x_2|^{n+d-1} \lambda_G(\mathrm{d}x_0) \right)\mu_{d,1}(\mathrm{d}G),
% \end{align*}
% where $\alpha_i$ is the angle between line $G$ and tangent hyperplane at point $x_i$. Noting that
% \[
%     \int\limits_{G \cap K} |x_0 - x_i|^{n+d-1} \lambda_G(\mathrm{d}x_0) = \int\limits_0^{|G \cap K|} x^{n+d-1} \mathrm{d}x = \frac{|G \cap K|^{n+d}}{n+d}
% \]
% finishes the proof.
% \end{proof}


Примененяя~\eqref{Zahle_rus} в случае многогранников, получаем следующий результат. 
\begin{thm}\label{thm4_rus}
Пусть $P$ --- выпуклый многогранник в $\mathbb{R}^d$,  $h(x_0, \ldots, x_l)$ --- измеримая функция, $l \leqslant d-1$. Тогда 

\begin{align*}
    &\int\limits_{(\partial P)^{l+1}} h(x_0,\ldots, x_l) \sigma_{\partial P}(\mathrm{d}x_0) \ldots \sigma_{\partial P}(\mathrm{d}x_l)  \\
    &=(l!)^{d-l}b_{d,l} 
     \sum_{\substack{(F_0, \ldots, F_l)\in\mathcal F^{l+1}(P)\\ \exists F_i \ne F_j}}
     \int\limits_{A_{d,l}}\int\limits_{E\cap F_0}\ldots
     \int\limits_{E\cap F_l} h(x_0, \ldots, x_l)  \\
     &\times
     |[x_0, \ldots, x_l]|^{d-l} \prod_{k=0}^{l}\|\mathrm P_E(n_P(x_k))\|^{-1} \lambda_{E \cap F_0 }(\mathrm{d}x_0)\ldots \lambda_{E \cap F_l}
     (\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E)  \\
     &+ (l!)^{d-l-1}b_{d-1,l}\cdot \sum_{F\in\mathcal F(P)} 
     \int\limits_{A_{F,l}}\int\limits_{(E \cap F)^{l+1}} h(x_0, \ldots, x_l)  \\
     &\times 
     |[x_0, \ldots, x_l]|^{d-l-1}\lambda_{E\cap F}(\mathrm{d}x_0)\ldots \lambda_{E \cap F}(\mathrm{d}x_l)\mu_{F,l}(\mathrm{d}E),  
\end{align*}
где  $n_P(x)$ обозначает внешнюю нормаль к $P$ в точке $x$, а  $\mathrm P_E$ есть ортогональная проекция на плоскость $E$.
\end{thm}


% Applying~\eqref{Zahle} to the polytopes gives the following result.
% \begin{thm}\label{thm4}
% Let $P$ be a convex polytope in $\mathbb{R}^d$ and let $h(x_0, \ldots, x_l)$ be a continuous function, $l \leqslant d-1$. Then 

% \begin{align*}
%     &\int\limits_{(\partial P)^{l+1}} h(x_0,\ldots, x_l) \sigma_{\partial P}(\mathrm{d}x_0) \ldots \sigma_{\partial P}(\mathrm{d}x_l)  \\
%     &=(l!)^{d-l}b_{d,l} 
%      \sum_{\substack{(F_0, \ldots, F_l)\in\mathcal F^{l+1}(P)\\ \exists F_i \ne F_j}}
%      \int\limits_{A_{d,l}}\int\limits_{E\cap F_0}\ldots
%      \int\limits_{E\cap F_l} h(x_0, \ldots, x_l)  \\
%      &\times
%      |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l} \prod_{k=0}^{l}\|\mathrm P_E(n_P(x_k))\|^{-1} \lambda_{E \cap F_0 }(\mathrm{d}x_0)\ldots \lambda_{E \cap F_l}
%      (\mathrm{d}x_l)\mu_{d,l}(\mathrm{d}E)  \\
%      &+ (l!)^{d-l-1}b_{d-1,l}\cdot \sum_{F\in\mathcal F(P)} 
%      \int\limits_{A_{F,l}}\int\limits_{(E \cap F)^{l+1}} h(x_0, \ldots, x_l)  \\
%      &\times 
%      |\mathrm{conv}(x_0, \ldots, x_l)|^{d-l-1}\lambda_{E\cap F}(\mathrm{d}x_0)\ldots \lambda_{E \cap F}(\mathrm{d}x_l)\mu_{F,l}(\mathrm{d}E),  
% \end{align*}
% where $n_P(x)$ denotes the outer unit normal vector of $P$ at $x$ and $\mathrm P_E$ is the orthogonal projection onto the hyperplane $E$.
% \end{thm}



Работа организована следующим образом. В разделах \ref{prf} и \ref{APprf} приведены доказательства Теоремы~\ref{thm1} и Теоремы~\ref{thm2}, далее приведено доказательство Теоремы~\ref{thm3} В разделе \ref{NewZahle}. Доказательство Теоремы~\ref{thm4} приводится в  разделе \ref{Zahlepoly}. 
